Does Learning from Decentralized Non-IID Unlabeled Data Benefit from Self Supervision?

Decentralized learning has been advocated and widely deployed to make efficient use of distributed datasets, with an extensive focus on supervised learning (SL) problems. Unfortunately, the majority of real-world data are unlabeled and can be highly heterogeneous across sources. In this work, we carefully study decentralized learning with unlabeled data through the lens of self-supervised learning (SSL), specifically contrastive visual representation learning. We study the effectiveness of a range of contrastive learning algorithms under decentralized learning settings, on relatively large-scale datasets including ImageNet-100, MS-COCO, and a new real-world robotic warehouse dataset. Our experiments show that the decentralized SSL (Dec-SSL) approach is robust to the heterogeneity of decentralized datasets, and learns useful representation for object classification, detection, and segmentation tasks. This robustness makes it possible to significantly reduce communication and reduce the participation ratio of data sources with only minimal drops in performance. Interestingly, using the same amount of data, the representation learned by Dec-SSL can not only perform on par with that learned by centralized SSL which requires communication and excessive data storage costs, but also sometimes outperform representations extracted from decentralized SL which requires extra knowledge about the data labels. Finally, we provide theoretical insights into understanding why data heterogeneity is less of a concern for Dec-SSL objectives, and introduce feature alignment and clustering techniques to develop a new Dec-SSL algorithm that further improves the performance, in the face of highly non-IID data. Our study presents positive evidence to embrace unlabeled data in decentralized learning, and we hope to provide new insights into whether and why decentralized SSL is effective.

==> experiments.tex <==
 
 \section{Overview of Our Study}\label{sec:experiment}
% Our study focuses on three dimensions of decentralized self-supervised learning: (i) different notions of distribution shift; (ii) different ML datasets/applications/models; (iii) different decentralized learning and self-supervised learning algorithms. We conduct experiments on standard datasets such as CIFAR\citep{krizhevsky2009cifar}, ImageNet\citep{krizhevsky2012imagenet,tian2020contrastive}, and a real-world Amazon dataset (See Figure \ref{fig:amazon_distribution_vis}).  

\lirui{to trim down and move to appendix a bit.} To clarify the experiment protocols, we separate the pipeline into \textbf{representation learning} (pretraining phase) and \textbf{downstream evaluation}  (evaluation phase). The pretraining phase often consists of standard self-supervised pretraining algorithms or supervised learning algorithms deployed on multiple unlabeled data sources, and the goal is to learn a shared representation network that performs well on various downstream tasks for the local data sources. For \textbf{ Dec-SSL}, we use \texttt{FedAvg}  \citep{mcmahan2017communication} with SimCLR \citep{chen2020simple} as the default decentralized self-supervised learning method. We also compare with cases where we have access to labels. First by default, we evaluate the baseline algorithm decentralized supervised learning, where we use \texttt{FedAvg} for end-to-end classification on the decentralized labeled data, denoted as \textbf{ Dec-SL}. To make a fair comparison with Dec-SSL on pretraining, we also make use of the representation learned from decentralized supervised learning -- we train supervised learning with \texttt{FedAvg}, and then use the feature extractor network as the backbone for downstream tasks. We denote this process as as \textbf{ Dec-SLRep}\lirui{do we need an even clearer definition?}. 


 The downstream evaluation phase aims to evaluate the representation  either from Dec-SSL or Dec-SLRep on a centralized fashion. We consider two protocols in the evaluation phase: \textbf{linear probing for image classification} \citep{zhang2016colorful} and \textbf{ fine-tuning for object detection/segmentation}  \citep{he2020momentum,doersch2015unsupervised}. For classification, we train linear classifier on top of the frozen pre-trained network and evaluate the top-1 classification accuracy. For object detection/segmentation, we fine-tune the network by using the pre-trained weights as initialization and training in an end-to-end fashion, and then we evaluate the mean Average Precision (mAP) metric. Downstream tasks are performed on balanced centralized train and test dataset from the same data distributions. Please refer to Appendix \S\ref{appendix:impl} for more implementation details and Table \ref{tab:experiment_setup} for a summary of experiment setups.

% \subsection{Data  heterogeneity and distribution shift \lirui{Discuss}}

% Classical machine learning, especially supervised learning, involves the distribution of both features  $x$ and  labels $y$. We start with distribution shift that describes how two distributions are different. In particular, distribution  shift can be usually categorized as  \textit{quantity skew, label distribution skew, input distribution skew, feature skew}  \citep{hsieh2020non}.\kz{do we want to explain them or not? if not, maybe not include?}  The distribution mismatch problem is a fundamental problem for inference and is of great interests to domain adaptation[cite], few-shot learning [cite], robust ML community[cite]\kz{why this sentence?}\lirui{maybe not put here, just want to make connection with other literature}. Data heterogeneity is a training problem for de-centralized learning, where the data naturally comes from different non-IID sources and poses challenges to standard learning procedure. 

% \kz{re-wrote the 1st paragraph as follows (pls read the compare, everything is serving for ``dec-SSL'', not the other way around):} In traditional machine learning, especially supervised learning, both the features $x$, the labels $y$, and/or the conditional distribution between them $p(y|x)$, can be heterogeneous. This heterogeneity has posed significant challenges in decentralized machine learning in general \citep{hsieh2020non}.The datasets used in decentralized learning, which are usually generated at different devices and locations, are by nature {\it heterogeneous} and have posed significant challenges.. These types of heterogeneity  can also be viewed as the distribution shift across different data sources

% {Heterogeneity in decentralized learning is usually  categorized as  \textit{input heterogeneity, label distribution heterogeneity, and the heterogeneity in the relationships between the features and labels}, respectively  \citep{hsieh2020non}.} We create {\it label heterogeneity}  by distributing each user with different 
% proportion of classes; we construct these via either sampling from a Dirichlet process or alternatively via skewness partitioning\citep{hsieh2020non}. We also create \textit{input heterogeneity} by leveraging the feature space of a pre-trained network on the data. See Appendix \S \ref{Amazon Data}  for a real-world example and \S \ref{appendix:data_hetereneity} for more details on how we create data heterogeneity across data sources.  




% \kz{to change..} 
With extensive experiments and analysis on a linear setting, we seek to answer the following questions: 
 {(1)   Can decentralized SSL rival the performance of its centralized  counterpart, and handle the non-IIDness of decentralized unlabeled data? (2) Under the non-IID decentralized learning settings, does the representation extracted from SSL behave more robustly from SL when we vary communication and participation rates? (3) Can we propose additional remedies to mitigate other challenges when dealing with non-i.i.d data such as feature misalignment and multi-modality? Our hypothesis is that visual contrastive learning, whose objective is not particularly dependent on the $x$ to $y$ mappings, learns a relatively {\it uniform}  representation across  heterogeneous unlabeled datasets, thus leading to more efficient and robust  decentralized learning schemes. 
}


 
